Listenable Maps for Zero-Shot Audio Classifiers

Interpreting the decisions of deep learning models, including audio classifiers, is crucial for ensuring the transparency and trustworthiness of this technology. In this paper, we introduce LMAC-ZS (Listenable Maps for Audio Classifiers in the Zero-Shot context), which, to the best of our knowledge, is the first decoder-based post-hoc interpretation method for explaining the decisions of zero-shot audio classifiers. The proposed method utilizes a novel loss function that maximizes the faithfulness to the original similarity between a given text-and-audio pair. We provide an extensive evaluation using the Contrastive Language-Audio Pretraining (CLAP) model to showcase that our interpreter remains faithful to the decisions in a zero-shot classification context. Moreover, we qualitatively show that our method produces meaningful explanations that correlate well with different text prompts.

==> letsusetheotherfile <==
@article{clap,
  title={Clap: Learning audio concepts from natural language supervision},
  author={Elizalde, Benjamin and Deshmukh, Soham and Ismail, Mahmoud Al and Wang, Huaming},
  journal={arXiv preprint arXiv:2206.04769},
  year={2022}
}


@inproceedings{chen20vggsound,
    author       = "Honglie Chen and Weidi Xie and Andrea Vedaldi and Andrew Zisserman",
    title        = "{VGGSound}: A Large-scale Audio-Visual Dataset",
    booktitle    = "ICASSP",
    year         = "2020",
}

@inproceedings{piczak2015esc,
    title={{ESC}: Dataset for Environmental Sound Classification},
    author={Karol J. Piczak},
    booktitle={ACM MM},
    year={2015}
}
%booktitle={ACM International Conference on Multimedia},

@inproceedings{bang2021vibi, 
    title={Explaining A Black-box By Using A Deep Variational Information Bottleneck Approach},
    opt_volume={35}, 
    opt_number={13}, 
    booktitle={AAAI}, 
    author={Bang, Seojin and Xie, Pengtao and Lee, Heewook and Wu, Wei and Xing, Eric}, year={2021}, 
    pages={11396--11404}
}

@inproceedings{parekh2020flint,
    title={A Framework to Learn with Interpretation},
    author={Jayneel Parekh and Pavlo Mozharovskyi and Florence d'Alch{\'e}-Buc},
    booktitle={NeurIPS},
    year={2020}
}

@article{hoyer2004nmf,
    title={Non-negative matrix factorization with sparseness constraints},
    author={Hoyer, Patrik O},
    journal={Journal of Machine Learning Research (JMLR)},
    opt_volume={5},
    opt_number={9},
    year={2004}
}

@inproceedings{parekh2022l2i,
    title={Listen to Interpret: Post-hoc Interpretability for Audio Networks with {NMF}},
    author={Jayneel Parekh and Sanjeel Parekh and Pavlo Mozharovskyi and Florence d'Alch{\'e}-Buc and Ga{\"e}l Richard},
    booktitle={NeurIPS},
    year={2022},
}

@inproceedings{yeh2020completeness,
    author = {Yeh, Chih-Kuan and others},
    title = {On Completeness-Aware Concept-Based Explanations in Deep Neural Networks},
    year = {2020},
    booktitle = {NeurIPS},
}
%author = {Yeh, Chih-Kuan and Kim, Been and Arik, Sercan \"{O}. and Li, Chun-Liang and Pfister, Tomas and Ravikumar, Pradeep},

@inproceedings{liang2022multiviz,
    title={{MultiViz}: Towards Visualizing and Understanding Multimodal Models},
    author={Paul Pu Liang and Yiwei Lyu and Gunjan Chhablani and Nihal Jain and Zihao Deng and Xingbo Wang and Louis-Philippe Morency and Ruslan Salakhutdinov},
    year={2023},
    booktitle={ICLR}
}

@article{selvaraju2016gradcam,
  title={{Grad-CAM}: Visual Explanations from Deep Networks via Gradient-Based Localization},
  author={Selvaraju, Ramprasaath R. and others},
  journal={ICCV},
  year={2017},
  pages={618--626},
}
%journal={IEEE International Conference on Computer Vision (ICCV)}
%author={Selvaraju, Ramprasaath R. and Cogswell, Michael and Das, Abhishek and Vedantam, Ramakrishna and Parikh, Devi and Batra, Dhruv},

@inproceedings{kim2018tcav,
  title = 	 {Interpretability Beyond Feature Attribution: Quantitative Testing with Concept Activation Vectors ({TCAV})},
  author =       {Kim, Been and others},
  booktitle = 	 {ICML},
  pages = 	 {2668--2677},
  year = 	 {2018},
  opt_volume = 	 {80},
}
%author =       {Kim, Been and Wattenberg, Martin and Gilmer, Justin and Cai, Carrie and Wexler, James and Viegas, Fernanda and Sayres, Rory},

@inproceedings{ghorbani2019,
 author = {Ghorbani, Amirata and Wexler, James and Zou, James Y and Kim, Been},
 booktitle = {NeurIPS},
 pages = {},
 title = {Towards Automatic Concept-based Explanations},
 opt_volume = {32},
 year = {2019}
}

@article{paissan2023piq,
  title={Posthoc Interpretation via Quantization}, 
  author={Francesco Paissan and Cem Subakan and Mirco Ravanelli},
  year={2023},
  journal={arXiv preprint arXiv:2303.12659},
}

@inproceedings{ribeiro2018anchors,
    author = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
    title = {Anchors: High-Precision Model-Agnostic Explanations},
    year = {2018},
    booktitle = {AAAI},
}
%booktitle = {AAAI Conference on Artificial Intelligence and Innovative Applications of Artificial Intelligence Conference %and AAAI Symposium on Educational Advances in Artificial Intelligence},

@inproceedings{lundberg2017unified,
    author = {Lundberg, Scott M. and Lee, Su-In},
    title = {A Unified Approach to Interpreting Model Predictions},
    year = {2017},
    booktitle = {NeurIPS},
    pages = {4768--4777},
}

@inproceedings{ribeiro2016lime,
    author = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
    title = {"{W}hy Should I Trust You?": Explaining the Predictions of Any Classifier},
    year = {2016},
    booktitle = {ACM SIGKDD ICKDDM},
    pages = {1135--1144},
    numpages = {10},
}
%booktitle = {ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  
@article{montavon2018interpreting,
    title = {Methods for interpreting and understanding deep neural networks},
    journal = {Digital Signal Processing},
    opt_volume = {73},
    pages = {1--15},
    year = {2018},
    author = {Grégoire Montavon and Wojciech Samek and Klaus-Robert Müller},
}

@inproceedings{gilpin2018,
    author={Gilpin, Leilani H. and Bau, David and Yuan, Ben Z. and Bajwa, Ayesha and Specter, Michael and Kagal, Lalana},
    booktitle={IEEE International Conference on Data Science and Advanced Analytics (DSAA)}, 
    title={Explaining Explanations: An Overview of Interpretability of Machine Learning}, 
    year={2018},
    opt_volume={},
    opt_number={},
    pages={80--89},
}

@article{li2022interpretability,
    author = {Li, Xuhong and others},
    title = {Interpretable Deep Learning: Interpretation, Interpretability, Trustworthiness, and Beyond},
    year = {2022},
    opt_volume = {64},
    opt_number = {12},
    journal = {Knowl. Inf. Syst.},
    pages = {3197--3234},
}
%author = {Li, Xuhong and Xiong, Haoyi and Li, Xingjian and Wu, Xuanyu and Zhang, Xiao and Liu, Ji and Bian, Jiang and Dou, Dejing},

@article{parekh2023tackling,
  title={Tackling Interpretability in Audio Classification Networks with Non-negative Matrix Factorization},
  author={Jayneel Parekh and Sanjeel Parekh and Pavlo Mozharovskyi and Gaël Richard and Florence d'Alché-Buc},
  journal={arXiv preprint arXiv:2305.07132},
  year={2023}
}

@article{zhang2021survey,
  author={Zhang, Yu and Tiňo, Peter and Leonardis, Aleš and Tang, Ke},
  journal={IEEE Transactions on Emerging Topics in Computational Intelligence}, 
  title={A Survey on Neural Network Interpretability}, 
  year={2021},
  opt_volume={5},
  pages={726--742},
}

@inproceedings{zarei2022prototypical,
  author={Zarei, Mohammad Reza and Komeili, Majid},
  booktitle={IEEE ICIP}, 
  title={Interpretable Concept-Based Prototypical Networks for Few-Shot Learning}, 
  year={2022},
  opt_volume={},
  opt_number={},
  pages={4078--4082},
}
%booktitle={IEEE International Conference on Image Processing (ICIP)},

@inproceedings{jain2020learning,
    title = "{L}earning to Faithfully Rationalize by Construction",
    author = "Jain, Sarthak  and
      Wiegreffe, Sarah  and
      Pinter, Yuval  and
      Wallace, Byron C.",
    booktitle = "ACL",
    pages = "4459--4473",
    year = "2020"
}
%booktitle = "Annual Meeting of the Association for Computational Linguistics",

@inproceedings{yoon2018invase,
    title={{INVASE}: Instance-wise Variable Selection using Neural Networks},
    author={Jinsung Yoon and James Jordon and Mihaela van der Schaar},
    booktitle={ICLR},
    year={2019},
}

@inproceedings{lee2019functional,
    title={Functional Transparency for Structured Data: a Game-Theoretic Approach}, 
    author={Guang-He Lee and Wengong Jin and David Alvarez-Melis and Tommi S. Jaakkola},
    year={2019},
    booktitle={ICML},
}

@inproceedings{vaswani2017transformer,
    author = {Vaswani, Ashish and others},
    title = {Attention is All You Need},
    year = {2017},
    booktitle = {NeurIPS},
    pages = {6000--6010},
}
%author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, \L{}ukasz and Polosukhin, Illia},

@inproceedings{ravanelli2018sincnet,
    author = {Ravanelli, Mirco and Bengio, Yoshua},
    title = {Interpretable Convolutional Filters with {SincNet}},
    year = {2018},
    booktitle = {NeurIPS IRASL Workshop},
}
%booktitle = {NeurIPS Interpretability and Robustness in Audio, Speech, and Language Workshop},

@article{becker2018lrp,
  title={Interpreting and explaining deep neural networks for classification of audio signals},
  author={Becker, S{\"o}ren and Ackermann, Marcel and Lapuschkin, Sebastian and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  journal={arXiv preprint arXiv:1807.03418},
  year={2018}
}

@inproceedings{muckenhirn2019relevance,
  title={Understanding and Visualizing Raw Waveform-Based {CNN}s},
  author={Muckenhirn, Hannah and Abrol, Vinayak and Magimai-Doss, Mathew and Marcel, S{\'e}bastien},
  booktitle={Interspeech},
  pages={2345--2349},
  year={2019}
}

@inproceedings{sundararajan2017ig,
    author = {Sundararajan, Mukund and Taly, Ankur and Yan, Qiqi},
    title = {Axiomatic attribution for deep networks},
    year = {2017},
    booktitle = {ICML},
    pages = {3319--3328},
}
%booktitle = {International Conference on Machine Learning (ICML)}

@inproceedings{haunschmid2020audiolime,
  title={{audioLIME}: Listenable explanations using source separation},
  author={Haunschmid, Verena and Manilow, Ethan and Widmer, Gerhard},
  booktitle={ECML-PKDD},
  year={2020}
}

@article{zinemanas2021apnet,
  title={An Interpretable Deep Learning Model for Automatic Sound Classification},
  author={Zinemanas, Pablo and Rocamora, Mart{\'\i}n and Miron, Marius and Font, Frederic and Serra, Xavier},
  journal={Electronics},
  opt_volume={10},
  pages={850},
  year={2021},
}

@inproceedings{li2018protodnn,
  title={Deep learning for case-based reasoning through prototypes: A neural network that explains its predictions},
  author={Li, Oscar and Liu, Hao and Chen, Chaofan and Rudin, Cynthia},
  booktitle={AAAI},
  opt_volume={32},
  year={2018}
}
%booktitle={AAAI Conference on Artificial Intelligence},

@article{ravanelli2021speechbrain,
    author = {Mirco Ravanelli and others},
    title = {{SpeechBrain}: A General-Purpose Speech Toolkit},
    journal = {arXiv preprint arXiv:2106.04624},
    year = {2021},
}
%    author = {Mirco Ravanelli and Titouan Parcollet and Peter Plantinga and Aku Rouhe and Samuele Cornell and Loren Lugosch and Cem Subakan and Nauman Dawalatabad and Abdelwahab Heba and Jianyuan Zhong and Ju-Chieh Chou and Sung-Lin Yeh and Szu-Wei Fu and Chien-Feng Liao and Elena Rastorgueva and François Grondin and William Aris and Hwidong Na and Yan Gao and Renato De Mori and Yoshua Bengio},

@inproceedings{kingma2015adam,
  author    = {Diederik P. Kingma and Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  booktitle = {ICLR},
  year      = {2015},
}

@inproceedings{adebayo2018sanity,
    author = {Adebayo, Julius and Gilmer, Justin and Muelly, Michael and Goodfellow, Ian and Hardt, Moritz and Kim, Been},
    booktitle = {NeurIPS},
    title = {Sanity Checks for Saliency Maps},
    volume = {31},
    year = {2018}
}
